Curious Representation Learning for Embodied Intelligence

Self-supervised representation learning has achieved remarkable success in recent years. By subverting the need for supervised labels, such approaches are able to utilize the numerous unlabeled images that exist on the Internet and in photographic datasets. Yet to build truly intelligent agents, we must construct representation learning algorithms that can learn not only from datasets but also learn from environments. An agent in a natural environment will not typically be fed curated data. Instead, it must explore its environment to acquire the data it will learn from. We propose a framework, curious representation learning (CRL), which jointly learns a reinforcement learning policy and a visual representation model. The policy is trained to maximize the error of the representation learner, and in doing so is incentivized to explore its environment. At the same time, the learned representation becomes stronger and stronger as the policy feeds it ever harder data to learn from. Our learned representations enable promising transfer to downstream navigation tasks, performing better than or comparably to ImageNet pretraining without using any supervision at all. In addition, despite being trained in simulation, our learned representations can obtain interpretable results on real images. Code is available at https://yilundu.github.io/crl/.

==> figText/atari_curious.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/blank.png}
\end{center}
\caption{\small Comparison of number of tiles explored in a given scene under each of the our policy methods}
\label{fig:num_tiles}
\vspace{-10pt}
\end{figure}

==> figText/carla_table.tex <==
\begin{table}
\centering
\caption{Comparison of linear finetuning classification accuracy on images from Places in a trained ResNet50 model under different visual representation learning algorithms (rows) using data obtained RL policy trained on different objective (column) on the Carla Environment. Across all visual representation learning algorithms, we find that data obtained CRL leads to the best linear finetuning accuracy, by enabling synergistic interactions between both policy training and visual representation learning}
\begin{tabular}{lcc}
    \toprule
     -  & Random Actions  & CRL  \\
     \midrule
     RND & & \\
     Colorization & & \\
     Contrastive Colorization & & \\
    %  Contrastive Colorization Queue & & \\
    %  Contrastive Colorization Replay Buffer & & \\
    \bottomrule
\end{tabular}

\label{tbl:carla_table}
\end{table}

==> figText/crl_policy_model.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{5.5pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
    \toprule
     Environment  & \multicolumn{3}{c}{Policy}  & \multicolumn{3}{c}{Representation Model} \\
     Number & Autoencode & Colorization & RND & Autoencode & Colorization & RND \\
     \midrule
     1 & \textbf{0.748} (0.016) & 0.676 (0.022) & 0.672 (0.014) & \textbf{0.864} (0.014) & 0.746 (0.018) & 0.751 (0.024) \\
     10 & \textbf{0.794} (0.005) & 0.733 (0.010) & 0.746 (0.013) & \textbf{0.872} (0.002) & 0.742 (0.017) & 0.789 (0.020) \\
     100 & \textbf{0.811} (0.006) & 0.762 (0.007) & 0.810 (0.012) & \textbf{0.863} (0.013) & 0.767 (0.010) & 0.792 (0.020) \\
     1000 & \textbf{0.819} (0.011) & 0.747 (0.005) & 0.806 (0.011) & \textbf{0.855} (0.002) & 0.770 (0.002) & 0.793 (0.019) \\
    \bottomrule
\end{tabular}
}
\caption{\small Correspondence between both better representations in policies and representation learning models (RND = random network distillation) under CRL. Value evaluated across 3 different seeds with standard error in parentheses. These result show stronger visual representation learning algorithms give stronger visual representations in policies.}
\label{tbl:policy_model_correspondance}
\vspace{-10pt}
\end{table}


==> figText/doom_model_rep.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{Linear fine-tuning accuracy of a learned representation model using different policies on the ViZDoom environment. CRL leads to the highest fine-tuning accuracy and trains a policy that generate diverse data. We evaluate on environments consisting of either 1, 10, or 100 pre-generated maps and use the autoencoding objective for CRL. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
    \toprule
    Environment & \multicolumn{5}{c}{Data Gathering Policy} \\
    \midrule
     Fixed Maps  & Counts & Movement& Shooter  & Random &  CRL  \\
     & Based & Distance & Optimization & \\
     \midrule
     1 &  0.858  & 0.862  & 0.820  &  0.834  & \textbf{0.864}  \\
     10 & 0.865  & 0.862  & 0.851  &  0.855  & \textbf{0.872}  \\
     100 & 0.862  & 0.860  & 0.847 & 0.853  & \textbf{0.863} \\
    \bottomrule
\end{tabular}
% }

\label{tbl:doom_model_rep}
\end{table*}

==> figText/habitat_exploration_map.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/blank.png}
\end{center}
\caption{Exploration of CRL compared to the exloration behavior of a random policy. Our framework encourages policies to effectively explore the surrounding environments.}
\label{fig:habitat_exploration}

\end{figure}

==> figText/habitat_policy_model.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{\small Comparison of policy and model visual representations in Habitat under different visual representation learning objectives. Improved model visual representations enable better visual representations for the policy. }
\begin{tabular}{l|c|c}
    \toprule
    Learning Objective & \multicolumn{2}{c}{Representation Accuracy} \\
    \midrule
       & Policy Accuracy  & Model Accuracy \\
     \midrule
     RND & 0.0560 & 0.058\\
     Colorization & 0.0605 &  0.095\\
     Contrastive Colorization  & 0.0833 & 0.150 \\
    %  Colorization + Contrastive + Queue & & \\
    %  Colorization + Contrastive + Replay Buffer & & \\
    \bottomrule
\end{tabular}
\label{tbl:habitat_policy_model}
\vspace{-10pt}
\end{table}

==> figText/habitat_table.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{Linear fine-tuning classification accuracy on images from Places using learned representation model in Habitat. We compare the effect of the representation learning algorithm (rows) and the RL policy (columns) on the Habitat Environment. Across all visual representation learning algorithms, CRL leads to the best linear finetuning accuracy, by enabling synergistic interactions between both policy training and visual representation learning}
\begin{tabular}{l|c|c|c}
    \toprule
    Learning Objective & \multicolumn{3}{c}{Data Gathering Policy} \\
    \midrule
      & Random & PointNav & CRL  \\
     \midrule
     RND & 0.056 & 0.036 & \textbf{0.058}\\
     Colorization & 0.072 & 0.051 & \textbf{0.104} \\
     Contrastive  Colorization & 0.098 & 0.058 & \textbf{0.150} \\
    %  Contrastive + Colorization + Queue & & & \\
    %  Contrastive + Colorization + Replay Buffer & & & \\
    \bottomrule
\end{tabular}
\label{tbl:habitat_table}
\vspace{-10pt}
\end{table}

% \begin{tabular}{lcccccc}
%     \toprule
%      -  & Random Actions  & PointNav & CRL  \\
%      \midrule
%      RND & 0.086 & 0.175 & 0.193 & 0.164  & -  & -\\
%      Colorization & 0.211 & 0.1066 & 0.253 & 0.085 & 0.324  & 0.084 \\
%     \bottomrule
% \end{tabular}

==> figText/heatmap.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/heatmap.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Comparison of random policy with CRL (with autoencoding objective) on a randomly generated test level of VizDoom. CRL is able to explore diverse paths that explore several chambers.}
\label{fig:heatmap_doom}
\vspace{-20pt}
\end{figure}

==> figText/heatmap_habitat.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/heatmap_habitat.pdf}
\end{center}
\caption{Comparison of random policy with CRL (curious representation learning) on random house in Habitat. CRL (with contrastive colorization objective) is able to diversely explore the surrounding environment.}
\label{fig:heatmap_habitat}
\vspace{-10pt}

\end{figure}

==> figText/model_rep.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{5.5pt}
\centering

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
    \toprule
     Environment  & Counts & Movement& Shooter  & CRL & Random \\
     Number & Based & Distance & Optimization & & Policy \\
     \midrule
     1 &  0.858 (0.008) & 0.862 (0.003) & 0.820 (0.005) & \textbf{0.864} (0.014) & 0.834 (0.012)\\
     10 & 0.865 (0.006) & 0.862 (0.001) & 0.851 (0.004) & \textbf{0.872} (0.003) & 0.855 {0.002} \\
     100 & 0.862 (0.002) & 0.860 (0.001) & 0.847 (0.002) & \textbf{0.863} (0.002) & 0.853 (0.003) \\
    \bottomrule
\end{tabular}
}
\caption{\small Table of visual representations learned from an autoencoding model from data collected from different policies trained in different number of ViZDoom environment. CRL incentives the policy to generate diverse data that allows the best model representations across different environment numbers.}
\label{tbl:model_rep}
\vspace{-10pt}
\end{table}


==> figText/model_rep_graph.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.45\textwidth}
    \begin{center}
    \includegraphics[width=1.0\linewidth]{fig/doom_model_rep.pdf}
    \end{center}
    \caption{\small Plots of linear fine-tuning classification accuracy of a learned model under different policies for interacting and collecting data on the VizDoom environment. CRL leads to the highest fine-tuning accuracy across varying numbers of pre-generated maps}
    \label{fig:policy_rep_graph}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
   \begin{center}
%   \vspace{-10pt}
    \includegraphics[width=1.0\linewidth]{fig/habitat_model_rep.pdf}
    \end{center}
    \caption{\small Plots of linear fine-tuning classifications of learned models under different policies for interacting on the Habitat environment.}
    \label{fig:rep_scatter}
    \end{minipage}
\end{figure}

==> figText/nearest_neighbor_carla.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/nearest_neighbors_carla.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Illustration of nearest neighbors on outdoors scenes in Places of a CRL model trained on Carla compared to a random network. CRL enables learning on high level visual features that transfer to real scenes.}
\label{fig:nearest_neighbor_carla}
\vspace{-10pt}
\end{figure}

==> figText/nearest_neighbor_doom.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/nearest_neighbor_doom.pdf}
\end{center}
\caption{\small Illustration of nearest neighbors in ViZDoom of a CRL policy compared to a random network. Nearest neighbor in CRL space is able to cluster more visually similar images}
\label{fig:nearest_neighbor_doom}
\end{figure}

==> figText/nearest_neighbor_habitat.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/nearest_neighbor_places_habitat.pdf}
\end{center}
\caption{\small Illustration of nearest neighbors on room scene in Places of a CRL model trained on Habitat compared to a random network. CRL enables learning on high level visual features that enable transfer to real scene as seen in the beds in the last row.}
\label{fig:nearest_neighbor_habitat}
\vspace{-10pt}
\end{figure}

==> figText/objective_rep.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/objective_rep.pdf}
\end{center}
\caption{\small Plots of correlation of representation learning (as measured by classification accuracy) with reward on objective. (CB = Counts Based, MD = Movement Distance, SO = Shooter Optimization). Results evaluated on 10 training levels. There is a strong correlation between objective optimization and visual representation.}
\label{fig:objective_rep}
\end{figure}

==> figText/policy_rep.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5.5pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
    \toprule
     Environment  & Counts & Movement & Shooter  & \multicolumn{3}{c}{CRL} \\
     Number & Based  & Distance & Optimization  & Autoencode & Colorization & RND \\
     \midrule
     1 & \textbf{0.749} (0.028) & 0.717 (0.017) & 0.772 (0.019) & 0.748 (0.016) & 0.676 (0.022) & 0.672 (0.013) \\
     10 & 0.783 (0.046) & 0.780 (0.010) & 0.679 (0.025) & \textbf{0.794} (0.011) & 0.733 (0.010) & 0.746 (0.010) \\
     100 & \textbf{0.818} (0.019) & 0.778 (0.013) & 0.723 (0.010) & 0.811 (0.012) & 0.762 (0.007) & 0.810 (0.012) \\
     1000 & 0.623 (0.079) & \textbf{0.832} (0.002) & 0.763 (0.006) & 0.819 (0.021) & 0.747 (0.005) & 0.805 (0.012) \\
    \bottomrule
\end{tabular}
}
\caption{\small Comparison of visual representations learned in policies from CRL and other objectives. We find that CRL with an autoencoding objective consistently gives relatively good visual representations while other objective, such counts based may sporadically give better visual representation, but are not consistently across environments.}
\label{tbl:policy_rep}
\end{table}


==> figText/policy_rep_graph_joint_scatter.tex <==
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=1.0\linewidth]{fig/policy_eval_graph.pdf}
% \end{center}
% \caption{Plots of policy visual representations when trained under different objectives with different number of environments}
% \label{fig:policy_rep_graph}
% \end{figure}
\begin{figure}
    \centering
    \begin{minipage}{0.45\textwidth}
   \begin{center}
    \includegraphics[width=1.0\linewidth]{fig/rep_scatter.pdf}
    \end{center}

    \caption{\small Scatter plot of different policy / model visual representation obtained from different variations of \model  on Doom. Variations on \model are obtained by varying number of fixed maps, and algorithms. Across variation, there is a strong correlation between policy and model representations.}
    \label{fig:rep_scatter}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
    \begin{center}
    \includegraphics[width=1.0\linewidth]{fig/habitat_policy_model.pdf}
    \end{center}

    \caption{\small Plots of visual representations (as measured by linear fine-tuning on Places) of both learned model and policy under different algorithms for \model. There is improved visual representations in both models and policies with better visual representation learning algorithms.}
    \label{fig:policy_model_habitat}
    \end{minipage}
\vspace{-10pt}
\end{figure}

==> figText/rep_casual.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{5.5pt}
\centering
\begin{tabular}{lcccc}
    \toprule
     -  & AE & RND & CL & Random\\
     \midrule
     Training Reward & 47.63 & 15.61 & 29.69 & 19.61 \\
     Classification Performance & 0.7994 & 0.721 & 0.766 & 0.468 \\
    \bottomrule
\end{tabular}
\caption{\small Relative performance on the MD objective when using CRL initialized with curious policies with representation learning values indicated compared with random policy after 1M frames of training on the shooter objective with 10 environments. Better representation learning through curiosity leads to better performance on the shooter enviornment.}
\label{tbl:rep_casual}
\vspace{-10pt}
\end{table}


==> figText/rep_scatter.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/rep_scatter.pdf}
\end{center}
\caption{\small Plots of policy visual representations with model visual representation under CRL with environment numbers of 10, 100, 1000. There is a good correlation of policy representation with model representation}
\label{fig:rep_scatter}
\end{figure}

==> figText/representation_progress.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.5\textwidth}
    \begin{table}[H]
    \setlength{\tabcolsep}{5.5pt}
    \centering
    \begin{tabular}{lccc}
        \toprule
        Environment & Counts  & Movement & Shooter\\
        Number & Based & Distance & Opt. \\
        \midrule
        1 & 0.794  & 0.719 & 0.573 \\ 
        10 & 0.911 & 0.733  & 0.549\\
        100 & 0.970 & 0.922 & 0.647 \\
        1000 & 0.689  & 0.826 & 0.635\\
        \bottomrule
    \end{tabular}
    \caption{\small Correlation coefficient of measured representation accuracy and objectives (reward across different environment numbers in ViZDoom evaluate across 3 different seeds). P values are all in the 1e-6 - 1e-12 range.}
    \label{tbl:representation_progress}
    \end{table}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
    \begin{table}[H]
    \setlength{\tabcolsep}{5.5pt}
    \centering
    % \begin{tabular}{lcccc}
    %     \toprule
    %      -  & AE & RND & CL & Random\\
    %      \midrule
    %      Training Reward & 47.63 & 15.61 & 29.69 & 19.61 \\
    %      Classification Performance & 0.7994 & 0.721 & 0.766 & 0.468 \\
    %     \bottomrule
    % \end{tabular}
    
    \begin{tabular}{lcc}
    \toprule
     CRL & Training & Classification \\
     Model & Reward & Performance \\
     \midrule
     Autoencoding & 47.63 & 0.799\\
     RND & 15.61 & 0.721 \\
     Colorization & 29.69 & 0.766\\
     Random & 19.61 & 0.468\\
    \bottomrule
    \end{tabular}
    \caption{\small Relative performance on the Movement Distance (10 levels) objective when using CRL initialized with curious policies with different representation learning values indicated compared with random policy after 1M frames of training.}
    \label{tbl:rep_casual}
    \end{table}
    \end{minipage}
    \vspace{-10pt}
\end{figure}







==> figText/representation_vis.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/representation_vis.pdf}
\end{center}
\vspace{-15pt}
\caption{\small An visualization of objective optimization with corresponding perceptual representation learning on the maximum distance from origin objective with 10 environments.}
\label{fig:representation_vis}
\vspace{-15pt}
\end{figure}

==> figText/rl_performance.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{\small Comparison of different approaches towards learning visual representations and there net effect on performance. Model with pre-trained representations are learned on \gc{To do}}
\begin{tabular}{l|l|cccc}
    \toprule
   Task & Method Objective & \multicolumn{4}{c}{Metrics} \\
    \midrule
       &  & Distance to Goal & SPL & Success Rate  & Reward \\
     \midrule
     \multirow{4}{*}{Habitat} & From Scratch & \\
       & ST-DIM & \\
       & CURL \\
       & Ours  \\
      \midrule
      
       \multirow{4}{*}{ViZDoom} & From Scratch & \\
       & ST-DIM & \\
       & CURL \\
       & Ours  \\

    %  Colorization + Contrastive + Replay Buffer & & \\
    \bottomrule
\end{tabular}
\label{tbl:rl_performance}
\vspace{-10pt}
\end{table*}


==> figText/teaser.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/method_with_networks.pdf}
\end{center}
\caption{When put in a new world, we are able to actively explore and interact with our surroundings. Our framework enables our agents (diagramed above) to actively interact, explore, and learn to represent their surrounding environment without any supervision. We show that we are able to learn effective visual representations of real images from observations purely actively gathered by our agent in both Habitat and Carla simulators. \gc{To do: to small}}
\label{fig:teaser}
\vspace{-20pt}
\end{figure}

==> text/experimental_setup.tex <==
\section{Experiment Setup}
\label{sect:experiment}
To evaluate visual representation learning and policy performance, we use four different sets of simulated environments. This section describes the details of the environment, experimental setup and architecture, and baselines.

\myparagraph{Environments:}
We use the following three different environments for evaluation:
\begin{enumerate}
    \item \textbf{ViZDoom:} The first environment we evaluate on is the ViZDoom environment \citep{kempka2016vizdoom}, based off the video game Doom. We use the level generator Oblige to generate new maps, with details in the appendix. Agents are spawned in a world with over ten rooms, random monsters, and stage hazards.  Agents have the ability to move forward, backwards, left and right, turn left and right, attack, speed, and interact with different objects.
    \item \textbf{Habitat:} The second environment we evaluate on is the Habitat environment \citep{habitat19arxiv}. We consider the Matterport \citep{chang2017matterport3d} and Gibson \citep{xia2018gibson} splits of the dataset, which consist of photorealistic scans on houses. The action space of the agent consists of 3 different movements, turn left, turn right, and move forward. To enable more effective navigation, in action of the agent is repeated twice. Agents are randomly spawned in a location in the house, with each episode terminated after 1000 actions.
    \item \textbf{Carla:} The third environment we evaluate on is the Carla environment \citep{dosovitskiy2017carla}, which consists of a self-driving simulation of cars The action space of the agent consists of 14 discrete actions corresponding to different possible combinations of steer, throttle and brake. Each episode is terminated upon collision with either the surrounding lane barriers or different pedestrians.
\end{enumerate}

\myparagraph{Training Details:} To train RL policies, on both Habitat and Carla environments, we utilize input images of size 224 by 224 and input images of size 168 by 168 by ViZDoom. We train with 8 environments in parallel for both Habitat and ViZDoom, and 4 environments in parallel for the Carla environment (due to computational restrictions). We train using the Adam Optimizer \citep{Kingma2015Adam} with learning rate 2e-4. We utilize a discount factor 0.99 and an entropy coefficient of 0.005. We optimize our policy 128 steps at a time. 


\myparagraph{Model Architectures:} For both Habitat and Carla environments, we use a ResNet50 \citep{He2015Deep} backbone architecture for the visual representation model. We different variants of residual networks for all other policies and visual representations across environments. For policies, we add a LSTM cell to the ResNet representation before decoding to value and policy predictions. To remove batch dependence we utilize layer normalization \citep{ba2016layer} in each residual layer as opposed to batch normalization \citep{Ioffe2015Batch}. We provide architectural details in the supplement. 

% For visual representation learning, we add different heads to backbone ResNet50, with a linear projection of 128 dimension for contrastive losses, and two fully connected layers of 512 hidden units for colorization. For the RL policy, we add a linear projection to 256 into a LSTM, which then decodes both values and actions.   For Atari environments, in line with previous works, we utilize the architecture from \citep{Mnih2013Playing} for our RL policy, and a network with two different residual blocks as our visual representation learning model. 

\myparagraph{Visual Representation Algorithms:} We use the following 4 different visual representation learning algorithms:
\begin{enumerate}
    \item \textbf{RND}: Random Network Distillation \citep{burda2018exploration} was originally proposed as a method to train curiosity model by using the error of a trained model in predicting the features of another random network as the intrinisic reward to a policy. Under our framework, we can treat this loss error is our visual representation learning loss. 
    \item \textbf{Autoencoding}: Auto-encoding corresponds to reconstructing an observation between an encoder and decoder network through a low dimensional bottleneck. After training through auto-encoding, we use the encoder as a visual representation learning model.
    \item \textbf{Colorization}: Colorization \citep{Zhang2016Colorful} predicts the ab channels of an image given the L channel
    \item \textbf{Contrastive Colorization}: Contrastive Colorization \citep{tian2019contrastive} seeks to maximize the mutual information between L and ab channels by contrasting ab channels from other images. 
\end{enumerate}
We include details of the heads and algorithms used for each visual representation learning algorithm in the supplement.

% We consider two different baselines for interactive policies in a environment. First we consider a random agent, which outputs random actions at each time point. Furthermore, in the Habitat environment, we consider an agent trained on the PointNav task, in when an agent is instructed to reach a goal destination. For visual representation learning we compare with baselines based of colorization and cross col 

\myparagraph{Visual Representation Evaluation:} To evaluate visual representation learning models, we use the standard practice of linear finetuning for classification on a frozen representation of the network \citep{Zhang2016Colorful}. We use the Adam optimizer to finetune linear weights with learning rate equal to 2e-4. We provide details about chosen frozen architectures in the supplement.

